Probing Left-handed Heavy Neutral Leptons on the Massive Vector Doublet Model

In the first part of this thesis, we consider an extension to the Standard Model composed by a Massive Vector Doublet under SU(2)L and a Left-handed Heavy Neutral Lepton. We study the production of these exotic leptons with a Same Flavor Opposite Sign standard lepton pair, and jets. We establish limits on the parameter space considering previous searches in this final state. After the limit definition, we study a modification on the event selection criteria in order to increase the possibility of probing these new particles at the Large Hadron Collider. Finally, we perform a parameter scan considering the new lepton as a dark matter candidate, identifying relevant regions on the parameter space for future studies.

==> Documents/ap1.tex <==
\chapter{Elements of Cosmology}\label{appa}
In this appendix, a general introduction to General Relativity is presented, as well as the main aspects of the $\Lambda$CDM model. To do so we are following the steps of Ref. \cite{cheng}.
\section{The structure of General Relativity}
The framework to describe the large scale structure of the Universe is General Relativity, which is a theory that associates the curvature of space-time with the energy and momentum distribution. The formulation of the theory begins with the metric tensor, $g_{\mu\nu}$. With this quantity we define the Levi-Civita connection:
\begin{equation}\label{eq:connection}
    \Gamma_{\mu\nu}^\lambda =\frac{g^{\lambda\rho}}{2}[\partial_\nu g_{\mu\rho}+\partial_\mu g_{\nu\rho}-\partial_{\rho}g_{\mu\nu}]
\end{equation}
With this quantity, we can define the Riemann Tensor:
\begin{equation}\label{eq:curvature}
    R_{\lambda \alpha\beta}^\mu=\partial_\alpha \Gamma_{\lambda\beta}^\mu-\partial_\beta\Gamma_{\lambda\alpha}^\mu+\Gamma_{\nu\alpha}^\mu \Gamma_{\lambda \beta}^\nu-\Gamma_{\nu\beta}^\mu \Gamma_{\lambda \alpha}^\nu
\end{equation}
This tensor contains all the information about the curvature of space-time, but is complicated to work with it. The usual thing is to consider one of it's traces. Doing this we obtain the Ricci tensor:
\begin{equation}
    R_{\mu\nu}= R_{\mu \alpha\nu}^\alpha
\end{equation}
This can be even more reduced, considering the Ricci scalar:
\begin{equation}
    R=g^{\alpha\beta}R_{\alpha\beta}
\end{equation}
All of this is combined in the Einstein tensor:
\begin{equation}
    G_{\mu\nu}=R_{\mu\nu}-\frac{1}{2}g_{\mu\nu}R
\end{equation}
Now that we have a parametrization of curvature, we need to describe the distribution of matter and energy, this is done with the definition of the Energy-Momentum tensor, $T_{\mu\nu}$. With this considerations, we can present the Einstein Field Equations:
\begin{equation}
    R_{\mu\nu}-\frac{1}{2}g_{\mu\nu} R-\lambda g_{\mu\nu}=-8\pi G_NT_{\mu\nu}
\end{equation}
Where $\Lambda$ is the cosmological constant, a parameter introduced by hand and can be understood as the vacuum contribution to the energy.
\section{Modelling the Universe with General Relativity}
The currents observations of the large scale structure of the universe show that it is homogeneous and isotropic, and can be modelated by the following ansatz for the metric:
\begin{equation}
    \mathrm{d}s^2=-\mathrm{d}t^2+a^2(t)\left[\frac{\mathrm{d}r^2}{1-kr^2}+r^2\mathrm{d}(\mathrm{d}\theta^2+\sin^2\theta\mathrm{d}\phi^2)\right]
\end{equation}
This is called the Friedmann-Lemaitre-Robertson Walker(FLRW) metric. On the other side, the homogeneity assumption can be used to suppose that the universe behaves like an ideal fluid. The Energy-Momentum tensor for such a fluid has the following form:
\begin{equation}
    T^{\mu\nu}=\begin{pmatrix}\rho&0&0&0\\0&p&0&0\\0&0&p&0\\0&0&0&p\end{pmatrix}
\end{equation}
Where $\rho$ and $p$ are the energy density and pressure of the fluid, respectively. Introducing the FLRW metric and the Energy-Momentum tensor of a perfect fluid in the Einstein Field Equations produces the Friedmann equations:
\begin{equation}
    \begin{split}
        &\left(\frac{\dot{a}}{a}\right)^2+\frac{k}{a^2}=\frac{8\pi}{3}\rho+ \frac{\Lambda}{3}\\
        &\left(\frac{\ddot{a}}{a}\right)=-\frac{4\pi}{3}(\rho+3p) +\frac{\Lambda}{3}
    \end{split}
\end{equation}
These equations describe the evolution of the Universe, and the first one is used to build the Standard Model of Cosmology, also known as $\Lambda$CDM Model.





==> Documents/ap2.tex <==
\chapter{Second appendix}


